Adaptable Recovery Behaviors in Robotics: A Behavior Trees and Motion Generators(BTMG) Approach for Failure Management

In dynamic operational environments, particularly in collaborative robotics, the inevitability of failures necessitates robust and adaptable recovery strategies. Traditional automated recovery strategies, while effective for predefined scenarios, often lack the flexibility required for on-the-fly task management and adaptation to expected failures. Addressing this gap, we propose a novel approach that models recovery behaviors as adaptable robotic skills, leveraging the Behavior Trees and Motion Generators~(BTMG) framework for policy representation. This approach distinguishes itself by employing reinforcement learning~(RL) to dynamically refine recovery behavior parameters, enabling a tailored response to a wide array of failure scenarios with minimal human intervention. We assess our methodology through a series of progressively challenging scenarios within a peg-in-a-hole task, demonstrating the approach's effectiveness in enhancing operational efficiency and task success rates in collaborative robotics settings. We validate our approach using a dual-arm KUKA robot.

==> abstract.tex <==
The ability to learn new tasks and quickly adapt to different variations and dimensions is an important attribute in agile robotics. In previous work, we have explored Behavior Trees and Motion Generators BTMGs) as a robot arm policy representation to facilitate the learning and execution of assembly tasks. The current implementation of the BTMGs for a specific task may not be robust to the changes in the environment and  may not generalize well to different variations of tasks. To address this limitation, we propose to extend the BTMG policy representation by learning a modeling function that maps task variations to BTMG parameters. To achieve this, we first train a Gaussian process to predict performance measure or reward that takes BTMG parameters and task variations as input. We also train a classifier to check the feasibility of the predicted policy. Subsequently, we optimize the performance measure over BTMG parameters for a fixed task variation.
To demonstrate the effectiveness of our proposed approach, we conducted experimental evaluations on push and obstacle avoidance tasks in simulation and also performed physical experiments using a \textit{KUKA iiwa} robot. Furthermore, we compared the performance of our approach with four baseline methods.
